Inexact Sequential Quadratic Optimization with Penalty Parameter Updates Within the QP Solve: Extended Version

This paper focuses on the design of sequential quadratic optimization (commonly known as SQP) methods for solving large-scale nonlinear optimization problems. The most computationally demanding aspect of such an approach is the computation of the search direction during each iteration, for which we consider the use of matrix-free methods. In particular, we develop a method that requires an inexact solve of a single QP subproblem to establish the convergence of the overall SQP method. It is known that SQP methods can be plagued by poor behavior of the global convergence mechanism. To confront this issue, we propose the use of an exact penalty function with a dynamic penalty parameter updating strategy to be employed within the subproblem solver in such a way that the resulting search direction predicts progress toward both feasibility and optimality. We present our parameter updating strategy and prove that, under reasonable assumptions, the strategy does not modify the penalty parameter unnecessarily. We also discuss a matrix-free subproblem solver in which our updating strategy can be incorporated. We close the paper with a discussion of the results of numerical experiments that illustrate the benefits of our proposed techniques.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% macros.tex                                         %
%                                                    %
% Current version: Michael P. Friedlander            %
%                  Dept of Computer Science          %
%                  University of British Columbia    %
%                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% $Revision: 1.2 $ $Date: 2004-04-20 10:18:51-05 $
% 13 Mar 1999: Added Abract environment
% 11 May 2000: Added several theorem environments
% 08 Jun 2001: Deleted absract environment
% 09 Nov 2001: Using RequirePackage to load req'd packages
% 21 Mar 2004: Deleted lots of never-used macros.  Cleanup.
% 06 Jul 2005: Using mathbb instead of mathds.  Looks better.

%%%%%%%%%%%
%  Packages
%%%%%%%%%%%
\RequirePackage{amsmath}
\RequirePackage{amssymb}
%\RequirePackage{dsfont}

%%%%%%%%%%%%%%%%%%%
% -- AMSMATH tweak:
% Subassumptions environment similar to subequations.
%%%%%%%%%%%%%%%%%%%
\makeatletter
\newcounter{parenttheorem}%
\newenvironment{subassumptions}{%
  \refstepcounter{theorem}%
  \protected@edef\theparenttheorem{\thetheorem}%
  \setcounter{parenttheorem}{\value{theorem}}%
  \setcounter{theorem}{0}%
  \def\thetheorem{\theparenttheorem\normalfont\alph{theorem}}%
  \ignorespaces
}{%
  \setcounter{theorem}{\value{parenttheorem}}%
  \ignorespacesafterend
}
\makeatother

%%%%%%%%%%%%%%%%%%%
% BibTeX macro.  Taken from /usr/share/texmf/doc/bibtex/base/btxdoc.tex.
%%%%%%%%%%%%%%%%%%%
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\def\tild{\raisebox{-0.5ex}{\~{}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Minimize, maximize, subject to
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\minim{\mathop{\hbox{minimize}}}
\def\maxim{\mathop{\hbox{maximize}}}
\def\minimize#1{\displaystyle\minim_{#1}}
\def\maximize#1{\displaystyle\maxim_{#1}}
\def\st{\mathop{\hbox{subject to}}}
\def\argmin{\mathop{\hbox{arg\,min}}}
\def\argmax{\mathop{\hbox{arg\,max}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Max/Min Problems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\def\uncprob#1#2#3{\fbox
  {\begin{tabular*}{0.84\textwidth}
      {@{}l@{\extracolsep{\fill}}l@{\extracolsep{9pt}}l@{\extracolsep{\fill}}l@{}}
      #1 & $\minimize{#2}$ & $#3$ & $ $
    \end{tabular*}}}
\def\problem#1#2#3#4{\fbox
  {\begin{tabular*}{0.84\textwidth}
      {@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}l@{}}
      #1 & $\minimize{#2}$ & $#3$ & $ $ \\[5pt]
         & $\st          $ & $#4$ & $ $
    \end{tabular*}}}
\def\problemnb#1#2#3#4{
  {\begin{tabular*}{0.84\textwidth}
      {@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}l@{}}
      #1 & $\minimize{#2}$ & $#3$ & $ $ \\[5pt]
         & $\st          $ & $#4$ & $ $
    \end{tabular*}}}
\def\probwide#1#2#3#4{\fbox
  {\begin{tabular*}{.98\textwidth}
      {@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}l@{}}
      #1 & $\minimize{#2}$ & $#3$ & $ $ \\[5pt]
         & $\st          $ & $#4$ & $ $
    \end{tabular*}}}
\def\probnarrow#1#2#3#4{\fbox
  {\begin{tabular*}{0.7\paperwidth}
      {@{}l@{\extracolsep{\fill}}c@{\extracolsep{6pt}}l@{\extracolsep{\fill}}l@{}}
      #1 & $\minimize{#2}$ & $#3$ & $ $ \\[5pt]
         & $\st          $ & $#4$ & $ $
    \end{tabular*}}}
\makeatother

\def\innerprod#1#2{\langle #1,#2\rangle}
\def\dps\displaystyle
\def\clink#1{\mkern2mu\overline{\mkern-2mu c\mkern2mu}\mkern-2mu\k(#1)}
\def\ul#1{\underline{#1}}
\def\Real{\mathbb{R}}
\def\Symm{\mathbb{S}}
\def\Complex{\mathbb{C}}
\def\m{\phantom-}
%\def\eval#1#2{\left.#2\right|_{\alpha=#1}}
% Matrices and vectors
%\def\tmat#1#2{(\, #1 \ \ #2 \,)}
%\def\tmatt#1#2#3{(\, #1 \ \  #2 \ \  #3\,)}
%\def\tmattt#1#2#3#4{(\, #1 \ \  #2 \ \  #3 \ \  #4\,)}
%\def\mat#1#2{(\; #1 \quad #2 \;)}
%\def\matt#1#2#3{(\; #1 \quad #2 \quad #3\;)}
%\def\mattt#1#2#3#4{(\; #1 \quad #2 \quad #3 \quad #4\;)}
\def\pmat#1{\begin{pmatrix}#1\end{pmatrix}}
\def\bmat#1{\begin{bmatrix}#1\end{bmatrix}}
\def\comp#1#2{[#2]_{#1}}
\def\compi#1{[#1]_i}
\def\compj#1{[#1]_j}
%\def\defd{\raisebox{-.2ex}{$\stackrel{\mathrm{def}}{=}$}}
\def\defd{\mathrel{\mathop:}=} % As per Higham's ``Accuracy & Stability...''
\def\abs#1{|#1|}
\def\norm#1{\|#1\|}
\def\onenorm#1{\|#1\|_1}
\def\twonorm#1{\|#1\|_2}
\def\infnorm#1{\norm{#1}_\infty}
\def\blackslug{\hbox{\hskip 1pt \vrule width 4pt height 6pt depth 1.5pt
  \hskip 1pt}}
\def\cross{{\scriptscriptstyle\times}}
\def\cond{\hbox{\rm cond}}
\def\det{\mathop{\hbox{\rm det}}}
\def\diag{\operatorname{diag}}
\def\dim{\mathop{\hbox{\rm dim}}}  
\def\boundary{\mathop{\hbox{\rm bnd}}}
\def\interior{\mathop{\hbox{\rm int}}}
\def\Null{\mathop{\hbox{\rm null}}}
\def\rank{\mathop{\hbox{rank}}}
\def\op{\mathop{\hbox{\rm op}}}
\def\range{\mathop{\hbox{\rm range}}}
\def\sign{\operatorname{sign}}
\def\sgn{\operatorname{sgn}}
\def\Span{\mbox{\rm span}}
\def\trace{\mathop{\hbox{\rm trace}}}
\def\drop{^{\null}}
\def\float{fl}
\def\grad#1{\nabla_{#1}}
\def\Hess#1{\nabla^2_{#1}}
\def\one{\mathbf{1}}
\def\half{{\textstyle{\frac{1}{2}}}}
\def\third{{\textstyle{\frac{1}{3}}}}
\def\fourth{{\textstyle{\frac{1}{4}}}}
\def\inv{^{-1}}
\def\invsq{^{-2}}
\def\limk{\lim_{k\to\infty}}
\def\mystrut{\vrule height10.5pt depth5.5pt width0pt}
\def\spose#1{\hbox to 0pt{#1\hss}}
\def\sub#1{^{\null}_{#1}}
\def\text #1{\hbox{\quad#1\quad}}
\def\textt#1{\hbox{\qquad#1\qquad}}
\def\invT{^{-T}\!}
\def\T{^T\!}
\def\pT{^{+T}}
\def\xint{{x_{\rm int}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Fixed-size glue, only for math mode
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\pthinsp{\mskip  2   mu}    %           thin space
\def\pmedsp {\mskip  2.75mu}    %         medium space
\def\pthiksp{\mskip  3.5 mu}    %          thick space
\def\nthinsp{\mskip -2   mu}
\def\nmedsp {\mskip -2.75mu}
\def\nthiksp{\mskip -3.5 mu}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Specially lowered subscripts (see \sub above)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Asubk{A\sub{\nthinsp k}}
\def\Bsubk{B\sub{\nthinsp k}}
\def\Fsubk{F\sub{\nmedsp k}}
\def\Gsubk{G\sub{\nthinsp k}}
\def\Hsubk{H\sub{\nthinsp k}}
\def\HsubB{H\sub{\nthinsp  \scriptscriptstyle{B}}}
\def\HsubS{H\sub{\nthinsp  \scriptscriptstyle{S}}}
\def\HsubBS{H\sub{\nthinsp \scriptscriptstyle{BS}}}
\def\Hz{H\sub{\nthinsp \scriptscriptstyle{Z}}}
\def\Jsubk{J\sub{\nmedsp k}}
\def\Psubk{P\sub{\nthiksp k}}
\def\Qsubk{Q\sub{\nthinsp k}}
\def\Vsubk{V\sub{\nmedsp k}}
\def\Vsubone{V\sub{\nmedsp 1}}
\def\Vsubtwo{V\sub{\nmedsp 2}}
\def\Ysubk{Y\sub{\nmedsp k}}
\def\Wsubk{W\sub{\nthiksp k}}
\def\Zsubk{Z\sub{\nthinsp k}}
\def\Zsubi{Z\sub{\nthinsp i}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Subscripts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\submax{_{\max}}
\def\submin{_{\min}}
\def\subminus{_{\scriptscriptstyle -}}
\def\subplus {_{\scriptscriptstyle +}}

\def\A{_{\scriptscriptstyle A}}
\def\B{_{\scriptscriptstyle B}}
\def\C{_{\scriptscriptstyle C}}
\def\D{_{\scriptscriptstyle D}}
\def\E{_{\scriptscriptstyle E}}
\def\F{_{\scriptscriptstyle F}}
\def\G{_{\scriptscriptstyle G}}
\def\H{_{\scriptscriptstyle H}}
\def\I{_{\scriptscriptstyle I}}
\def\J{_{\scriptscriptstyle J}}
\def\K{_{\scriptscriptstyle K}}
\def\L{_{\scriptscriptstyle L}}
\def\M{_{\scriptscriptstyle M}}
\def\N{_{\scriptscriptstyle N}}
\def\O{_{\scriptscriptstyle O}}
\def\P{_{\scriptscriptstyle P}}
\def\Q{_{\scriptscriptstyle Q}}
\def\R{_{\scriptscriptstyle R}}
\def\U{_{\scriptscriptstyle U}}
\def\V{_{\scriptscriptstyle V}}
\def\W{_{\scriptscriptstyle W}}
\def\Y{_{\scriptscriptstyle Y}}
\def\Z{_{\scriptscriptstyle Z}}
\def\k{_k}
\def\kp#1{_{k+#1}}
\def\km#1{_{k-#1}}
\def\j{_j}
\def\jp#1{_{j+#1}}
\def\jm#1{_{j-#1}}
\def\subb{\B}
\def\subc{\C}
\def\subf{\F}
\def\subh{\H}
\def\subk{\K}
\def\subm{\M}
\def\subn{\N}
\def\subp{\P}
\def\subs{_{\scriptscriptstyle S}}
\def\subt{_{\scriptscriptstyle T}}
\def\subr{\R}
\def\subz{\Z}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  bars, hats, tildes  (\skew4 is the default)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\alphabar{\bar \alpha}
\def\alphahat{\skew3\hat \alpha}
\def\alphatilde{\skew3\tilde \alpha}
\def\betabar{\skew{2.8}\bar\beta}
\def\betahat{\skew{2.8}\hat\beta}
\def\betatilde{\skew{2.8}\tilde\beta}
\def\deltabar{\bar\delta}
\def\deltilde{\skew5\tilde \delta}
\def\deltatilde{\deltilde}
\def\etabar{\bar\eta}
\def\gammabar{\bar\gamma}
\def\lambar{\bar\lambda}
\def\lamhat{\skew{2.8}\hat \lambda}
\def\lambdahat{\lamhat}
\def\lambdatilde{\tilde{\lambda}}
\def\lambdabar{\bar \lambda}
\def\mubar{\skew3\bar \mu}
\def\muhat{\skew3\hat \mu}
\def\mutilde{\skew3\tilde\mu}
\def\nubar{\skew3\bar\nu}
\def\nuhat{\skew3\hat\nu}
\def\nutilde{\skew3\tilde\nu}
\def\omegabar{\bar\omega}
\def\omegahat{\skew3\hat\omega}
\def\omegatilde{\tilde\omega}
\def\phibar{\bar\phi}
\def\pibar{\bar\pi}
\def\pihat{\skew1\widehat \pi}
\def\sigmaB{\mkern 3mu\overline {\mkern-3mu\sigma\mkern 1mu}\mkern-1mu}
\def\sigmab{\mkern-2mu\underline{\mkern 2mu\sigma\mkern-3mu}\mkern 3mu}
\def\sigmabar{\bar\sigma}
\def\rhobar{\bar\rho}
\def\rhohat{\widehat\rho}
\def\taubar{\bar\tau}
\def\tautilde{\tilde\tau}
\def\tauhat{\hat\tau}
\def\thetabar{\bar\theta}
\def\xibar{\skew4\bar\xi}

\def\abar{\skew3\bar a}
\def\ahat{\skew2\widehat a}
\def\atilde{\skew2\widetilde a}
\def\Abar{\skew7\bar A}
\def\Ahat{\widehat A}
\def\Atilde{\widetilde A}
\def\bbar{\skew3\bar b}
\def\bhat{\skew2\widehat b}
\def\btilde{\skew2\widetilde b}
\def\Bbar{\bar B}
\def\Bhat{\widehat B}
\def\cbar{\skew3\bar c}
\def\chat{\skew3\widehat c}
\def\ctilde{\widetilde c}
\def\Cbar{\bar C}
\def\Chat{\widehat C}
\def\Ctilde{\widetilde C}
\def\dbar{\bar d}
\def\dhat{\widehat d}
\def\dtilde{\widetilde d}
\def\Dbar{\bar D}
\def\Dhat{\widehat D}
\def\Dtilde{\widetilde D}
\def\ehat{\skew3\widehat e}
\def\ebar{\bar e}
\def\Ebar{\bar E}
\def\Ehat{\widehat E}
\def\Etilde{\widetilde E}
\def\fbar{\bar f}
\def\fhat{\widehat f}
\def\ftilde{\widetilde f}
\def\Fbar{\bar F}
\def\Fhat{\widehat F}
\def\Ftilde{\widetilde F}
\def\gbar{\skew{4.3}\bar g}
\def\ghat{\skew{3}\widehat g}
\def\gtilde{\skew{4.5}\widetilde g}
\def\Gbar{\bar G}
\def\Ghat{\widehat G}
\def\hbar{\skew{4.2}\bar h}
\def\hhat{\skew2\widehat h}
\def\htilde{\skew3\widetilde h}
\def\Hbar{\skew5\bar H}
\def\Hhat{\widehat H}
\def\Htilde{\widetilde H}
\def\Ibar{\skew5\bar I}
\def\Itilde{\widetilde I}
\def\Jbar{\skew6\bar J}
\def\Jhat{\widehat J}
\def\Jtilde{\widetilde J}
\def\kbar{\skew{4.4}\bar k}
\def\Khat{\widehat K}
\def\Kbar{\skew{4.4}\bar K}
\def\Ktilde{\widetilde K}
\def\ellbar{\bar \ell}
\def\lhat{\skew2\widehat l}
\def\lbar{\skew2\bar l}
\def\Lbar{\skew{4.3}\bar L}
\def\Lhat{\widehat L}
\def\Ltilde{\widetilde L}
\def\mbar{\skew2\bar m}
\def\mhat{\widehat m}
\def\Mbar{\skew{4.4}\bar M}
\def\Mhat{\widehat M}
\def\Mtilde{\widetilde M}
\def\Nbar{\skew{4.4}\bar N}
\def\Ntilde{\widetilde N}
\def\nbar{\skew2\bar n}
\def\pbar{\skew2\bar p}
\def\phat{\skew2\widehat p}
\def\ptilde{\skew2\widetilde p}
\def\Pbar{\skew5\bar P}
\def\Phat{\widehat P}
\def\Ptilde{\skew5\widetilde P}
\def\qbar{\bar q}
\def\qhat{\skew2\widehat q}
\def\qtilde{\widetilde q}
\def\Qbar{\bar Q}
\def\Qhat{\widehat Q}
\def\Qtilde{\widetilde Q}
\def\rbar{\skew3\bar r}
\def\rhat{\skew3\widehat r}
\def\rtilde{\skew3\widetilde r}
\def\Rbar{\skew5\bar R}
\def\Rhat{\widehat R}
\def\Rtilde{\widetilde R}
\def\sbar{\bar s}
\def\shat{\widehat s}
\def\stilde{\widetilde s}
\def\Shat{\widehat S}
\def\Sbar{\skew2\bar S}
\def\tbar{\bar t}
\def\ttilde{\widetilde t}
\def\that{\widehat t}
\def\Tbar{\bar T}
\def\That{\widehat T}
\def\Ttilde{\widetilde T}
\def\ubar{\skew3\bar u}
\def\uhat{\skew3\widehat u}
\def\utilde{\skew3\widetilde u}
\def\Ubar{\skew2\bar U}
\def\Uhat{\widehat U}
\def\Utilde{\widetilde U}
\def\vbar{\skew3\bar v}
\def\vhat{\skew3\widehat v}
\def\vtilde{\skew3\widetilde v}
\def\Vbar{\skew2\bar V}
\def\Vhat{\widehat V}
\def\Vtilde{\widetilde V}
\def\wbar{\skew3\bar w}
\def\what{\skew3\widehat w}
\def\wtilde{\skew3\widetilde w}
\def\Wbar{\skew3\bar W}
\def\What{\widehat W}
\def\Wtilde{\widetilde W}
\def\xbar{\bar{x}}
\def\xhat{\skew{2.8}\widehat x}
\def\xtilde{\skew3\widetilde x}
\def\Xhat{\widehat X}
\def\ybar{\skew3\bar y}
\def\yhat{\skew2\widehat y}
\def\ytilde{\skew3\widetilde y}
\def\Ybar{\skew2\bar Y}
\def\Yhat{\widehat Y}
\def\zbar{\skew{2.8}\bar z}
\def\zhat{\skew{2.8}\widehat z}
\def\ztilde{\skew{2.8}\widetilde z}
\def\Zbar{\skew5\bar Z}
\def\Zhat{\widehat Z}
\def\Ztilde{\widetilde Z}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Stars
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\lamstar{\lambda^*}
\def\lamstark{\lambda^*\k}
\def\lambarstark{\lambar^*\k}
\def\pistar{\pi^*}
\def\pistark{\pi^*_k}
\def\rhostar{\rho^*}
\def\mustar{\mu^*}
\def\taustar{\tau^*}
\def\cstar{c^*}
\def\dstar{d^*}
\def\gstar{g^*}
\def\Jstar{J^*}
\def\pstar{p^*}
\def\rstar{r^*}
\def\rstark{r^*\k}
\def\vstar{v^*}
\def\vstark{v^*\k}
\def\wstar{w^*}
\def\wstark{w^*\k}
\def\xstar{x^*}
\def\xstarhatk{\hat x^*\k}
\def\xstark{x^*\k}
\def\xstarzero{x^*_0}
\def\xstarkm1{x^*\km1}
\def\ystar{y^*}
\def\ystarhatk{\hat y^*\k}
\def\ystark{y^*\k}
\def\ystarkm1{y^*\km1}
\def\zstar{z^*}
\def\zstark{z^*\k}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Math italic fonts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\mit{\mathit}
\def\Deltait{{\mit \Delta}}
\def\Gammait{{\mit \Gamma}}
\def\Lambdait{{\mit \Lambda}}
\def\Sigmait{{\mit \Sigma}}
\def\Lambarit{\skew5\bar{\mit \Lambda}}
\def\Omegait{{\mit \Omega}}
\def\Omegaitbar{\skew5\bar{\mit \Omega}}
\def\Thetait{{\mit \Theta}}
\def\Piitbar{\skew5\bar{\mit \Pi}}
\def\Piit{{\mit \Pi}}
\def\Phiit{{\mit \Phi}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Math calligraphy fonts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\lscr{\ell}
\def\Ascr{\mathcal{A}}
\def\Bscr{\mathcal{B}}
\def\Cscr{\mathcal{C}}
\def\Escr{\mathcal{E}}
\def\Fscr{\mathcal{F}}
\def\Dscr{\mathcal{D}}
\def\Iscr{\mathcal{I}}
\def\Jscr{\mathcal{J}}
\def\Kscr{\mathcal{K}}
\def\Lscr{\mathcal{L}}
\def\Mscr{\mathcal{M}}
\def\Nscr{\mathcal{N}}
\def\Oscr{\mathcal{O}}
\def\Pscr{\mathcal{P}}
\def\Qscr{\mathcal{Q}}
\def\Rscr{\mathcal{R}}
\def\Sscr{\mathcal{S}}
\def\Tscr{\mathcal{T}}
\def\Uscr{\mathcal{U}}
\def\Vscr{\mathcal{V}}
\def\Wscr{\mathcal{W}}
\def\Zscr{\mathcal{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Delta quantities
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\dd{\Deltait d}
\def\dx{\Deltait x}
\def\dy{\Deltait y}
\def\dz{\Deltait z}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Computer packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Matlab{\textsc{Matlab}}
\newcommand{\code}[1]{{\small#1}}
\def\KNOSSOS{\code{KNOSSOS}}
\def\MINOS  {\code{MINOS}}
\def\LANCE  {\code{LANCELOT}}
\def\SNOPT  {\code{SNOPT}}
\def\SLQP   {S$\ell_1$QP}
\def\QPSOL  {\code{QPSOL}}
\def\LUSOL  {\code{LUSOL}}
\def\LSSOL  {\code{LSSOL}}
\def\GAMS   {\code{GAMS}}
\def\AMPL   {\code{AMPL}}
\def\COPS   {\code{COPS}}
\def\CUTE   {\code{CUTE}}
\def\CUTEr  {\code{CUTEr}}
\def\ADIC   {\code{ADIC}}
\def\CONOPT {\code{CONOPT}}
\def\NEOS   {\code{NEOS}}
\def\cpp    {C\raisebox{0.1ex}{\hbox{\small++}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Sec{\S}
\def\seq#1{\ensuremath{\{#1\}}}
\newcommand{\e}[1]{e\raisebox{.2ex}{\tiny$#1$}} % scientific not. (e)
\newcommand{\ozgur}{{\"O}zg{\"u}r Y{\i}lmaz}  % Ozgur Yilmaz's name!
